TACLE: Task and Class-aware Exemplar-free Semi-supervised Class Incremental Learning

We propose a novel TACLE (TAsk and CLass-awarE) framework to address the relatively unexplored and challenging problem of exemplar-free semi-supervised class incremental learning. In this scenario, at each new task, the model has to learn new classes from both (few) labeled and unlabeled data without access to exemplars from previous classes. In addition to leveraging the capabilities of pre-trained models, TACLE proposes a novel task-adaptive threshold, thereby maximizing the utilization of the available unlabeled data as incremental learning progresses. Additionally, to enhance the performance of the under-represented classes within each task, we propose a class-aware weighted cross-entropy loss. We also exploit the unlabeled data for classifier alignment, which further enhances the model performance. Extensive experiments on benchmark datasets, namely CIFAR10, CIFAR100, and ImageNet-Subset100 demonstrate the effectiveness of the proposed TACLE framework. We further showcase its effectiveness when the unlabeled data is imbalanced and also for the extreme case of one labeled example per class.

==> Figures/algoTale.tex <==
% \SetKwComment{Comment}{/* }{ */}
 \SetKwComment{Comment}{\qquad }{}
\KwIn{$\{\Theta, \psi^{(1)}\} \leftarrow $ Intial model; \\
$\{\mathcal{D}^{(1)}, \mathcal{D}^{(2)},\ldots,\mathcal{D}^{(\mathcal{T})}\} \leftarrow $ Data stream}
$E_{s1} \leftarrow$ No. of epochs for stage 1; $E_{s2} \leftarrow$ No. of epochs for stage 2;

\For{$t \leftarrow 1$ to $\mathcal{T}$}{
  % $\mathcal{D}^{t} \in {\mathcal{D}_{l}^{(t)} \cup  \mathcal{D}_{ul}^{(t)}}$\\
  $\mathcal{D}_{l}^{(t)} = \{\mathbf{x}_{i}^{l}, y_{i}^{l}\}_{i=1}^{N_{l}^{(t)}}, \mathcal{D}_{ul}^{(t)} = \{\mathbf{x}_{i}^{ul}\}_{i=1}^{N_{ul}^{(t)}}$\\
  % $\mathbf{x}_{i}^{l} \leftarrow$ labeled sample\\
  % $\mathbf{x}_{i}^{ul} \leftarrow$ unlabeled sample, $\mathbf{\hat{x}}_{i}^{ul} \leftarrow$ strongly augmented unlabeled sample\\
  % $w_{i}^{l} \leftarrow 1,  w_{i}^{ul} \leftarrow 1$ $\forall$ $i$\\
  % $\gamma_{d}^{t} \leftarrow \frac{\alpha}{1+e^{\alpha t}} + \beta$\\
  
  $\# Stage $ 1: {Feature Representation Learning}\\
  \For{$e_{s1} \leftarrow 1$ to $E_{s1}$}{
     $\mathbf{x} \leftarrow [\mathbf{x}_{i}^{l}, \mathbf{x}_{i}^{ul}, \mathbf{\hat{x}}_{i}^{ul}]$\\
     $\mathbf{p}_{i}^{l}$, $\mathbf{p}_{i}^{ul}$, $\mathbf{\hat{p}}_{i}^{ul} \leftarrow \Theta(\psi^{(t)}(x))$\\
     $\mathcal{L}_{stage1} \leftarrow \mathcal{L}_{s}(x_{i}^{l}, y_{i}^{l}) \cdot w_{i}^{l} + \mathcal{L}_{us}(x_{i}^{ul}) \cdot w_{i}^{ul}$\\
     Update parameters of $\Theta \And \psi^{(t)}$ using loss $\mathcal{L}_{stage1}$\\
     $\zeta \leftarrow \mathcal{D}_{ul}^{(t)}, \gamma_{d}^{t}$\\
     Update $w_{i}^{l} \And w_{i}^{l}$ using normalized $\zeta$ i.e., $\bar{\zeta}$\\  
  }\\


  $\# Stage $ 2: Classifier Alignment\\
    $\tilde{\mathcal{D}}_{ul}^{(t)}\leftarrow \mathcal{D}_{ul}^{(t)}, \gamma_{d}^{t}$\\
    $\mu_{t}, \Sigma_{t} \leftarrow \mathcal{D}_{l}^{(t)}  \cup \tilde{\mathcal{D}}_{ul}^{(t)} $\\
    $\tilde{\mu_{t}}, \tilde{\Sigma_{t}} \leftarrow [(\mu_{1}, \Sigma_{1}), (\mu_{2}, \Sigma_{2}) \dots (\mu_{t}, \Sigma_{t})]$\\
    \For{$e_{s2} \leftarrow 1$ to $E_{s2}$}{
     $\mathcal{L}_{ca} \leftarrow \tilde{\mu_{t}}, \tilde{\Sigma_{t}}$\\
     Update $\psi^{(1:t)}$ using $\mathcal{L}_{ca}$\\
    
  }
}


==> Figures/motivation_plot.tex <==
\begin{tikzpicture}[scale=1]
\definecolor{color0}{HTML}{F0F8FF}
\definecolor{color1}{HTML}{778899}
\definecolor{color2}{HTML}{696969}

\begin{groupplot}[group style={group name =GSS CIL experiments all datasets,group size=2 by 1,horizontal sep = 1.5cm,vertical sep = 1.5cm,}, title style={anchor=north, yshift=2.5ex} ]
  \nextgroupplot[
  tick align=outside,title={(a) CIFAR10},
    xlabel={Tasks},
    ylabel={MoMp},
    xtick={1,2,3,4,5},
    xticklabels={1,2,3,4,5},
    ymin=0.5, ymax=1.1,
    legend style={at={(0.5,-0.15)}, anchor=north, legend columns=-1},
    axis background/.style={fill=color0},
    width=5cm, height=3cm,
   x label style={at={(axis description cs:0.5,-0.0)},anchor=north},
    y label style={at={(axis description cs:0.05,0.5)},anchor=north},
    ]
    
    % Scatter plot
    \addplot[very thick, color= color1, mark=*,
      mark options={scale=1, color=color2},
      ] coordinates {
        (1, 0.9863)
        (2, 0.8642)
        (3, 0.81)
        (4, 0.83)
        (5, 0.64)
      };

    \nextgroupplot[
    tick align=outside,title={(a) CIFAR100},
    xlabel={Tasks},
    ylabel={MoMp},
    xtick={1,2,3,4,5,6,7,8,9,10},
    xticklabels={1,2,3,4,5,6,7,8,9,10},
    ymin=0.5, ymax=1.1,
    legend style={at={(0.5,-0.15)}, anchor=north, legend columns=-1},
    axis background/.style={fill=color0},
    width=5cm, height=3cm,
   x label style={at={(axis description cs:0.5,-0.0)},anchor=north},
    y label style={at={(axis description cs:0.05,0.5)},anchor=north},
    ]
    
    % Scatter plot
    \addplot[very thick, color= color1, mark=*,
      mark options={scale=1, color=color2},
      ] coordinates {
        (1, 0.9406)
        (2, 0.80)
        (3, 0.81)
        (4, 0.78)
        (5, 0.75)
        (6, 0.67)
        (7, 0.7)
        (8, 0.69)
        (9, 0.72)
        (10, 0.62)
      };
    % Add legend
    % \legend{Accuracy}
  % \end{axis}
  \end{groupplot}
\end{tikzpicture}

==> intro.tex <==
% \section{Introduction}
Recently, incremental or continual learning has become an important research direction due to its wide applicability in the field of artificial intelligence, especially in real-time scenarios where models need to adapt to new data continuously. Unlike traditional learning approach, incremental learning addresses the practical limitations of collecting all data at once and potential privacy concerns where only the model, not the training data, is accessible. But the major challenge faced by modern deep learning models when dealing with continuous data is catastrophic forgetting, where previously learned knowledge is overwritten as the model adapts to new information. Among various settings in incremental learning, class incremental learning has gained popularity due to its challenging nature and wide applicability in real-time scenarios.

In class incremental learning, the model is initially trained on a set of base classes and is subsequently updated when a new set of classes becomes available. This approach enables the model to expand its knowledge and capabilities by incorporating additional classes into its existing knowledge, allowing it to classify all the classes encountered so far. In the literature, the process of adding a set of new classes to a model is commonly referred to as a \textit{task}. Before transitioning to a new task, the most widely used technique to mitigate catastrophic forgetting is to save some samples from old tasks, often referred to as \textit{exemplars}. The number of exemplars stored in the storage buffer significantly affects the performance of class incremental learning algorithms. Another major assumption  in class-incremental learning (CIL) is abundant data availability at each task. However, large amounts of labeled data may be impractical or infeasible to collect in real-world scenarios. Few-Shot Class-Incremental Learning (FSCIL) addresses this by leveraging limited labeled data, attracting significant research attention. Our work focuses on Semi-Supervised Class-Incremental Learning (SS-CIL), where we have access to a large amount of unlabeled data alongside few labeled samples per task, along with we enforced the exemplar-free constraint where we dont have access to any data samples from the old tasks. Figure [] shows the clear distinguishes between CIL, SS-CIL and exemplar-free SS-CIL scenarios. SS-CIL differs slightly from traditional semi-supervised learning (SSL), where access to both labeled and unlabeled data occurs within only a single task. In SS-CIL, labeled and unlabeled data are encountered in a task-wise manner, making the problem more challenging.

Foundation models have recently played a significant role in modern computer vision applications. In a recent study [], these models were employed for CIL also refererd as slow learner for classifier alignment (SLCA). However, directly applying foundation models to SS-CIL setups may not be effective. To analyze the impact of foundation models in SS-CIL, we incorporated the popular threshold-based semi-supervised learning (SSL) approach known as FixMatch[] with SLCA. FixMatch is an algorithm where, if the confidence of unlabeled samples crosses a predefined threshold (typically 0.95), the unlabeled sample is trained with the pseudo-label of that class. While this approach effectively learns from unlabeled data, in the SS-CIL setting, a fixed threshold may not be effective. The number of classes increases with each task, impact the confidence distribution of unlabeled data. To analyze this confidence variation, we plotted the mean of maximum probabilities (MoMP) of unlabeled data after each task across various datasets. This will give us the idea of on an average what is the maximum confidence of unlabeled data. From figure~\ref{fig:momp_vs_tasks} empirically  we observed that the MoMP value reduced as tasks increased. Maintaining a fixed hard threshold may not effectively leverage learning from the unlabeled data in this dynamic setting. Based on this observation we proposed a \textit{task-wise adaptive threshold} to effectively utilize the unlabeled data. 

Additionally, there is a notable imbalance in the unlabeled data that surpasses the threshold. To address this issue, we introduced a \textit{data-aware weighted cross-entropy loss} to enhance performance on under-represented classes. Furthermore, we exploit the unlabeled data into the foundation model's classifier alignment process, further boosting performance in the context of semi-supervised class incremental learning (SS-CIL). To the best of our knowledge, this is the first work addressing the exemplar-free SS-CIL setting in the literature. It leverages foundation models to effectively tackle the challenges associated with SS-CIL. Extensive experiments conducted on various datasets, including CIFAR-10, CIFAR-100, and ImageNet-Subset, demonstrate the effectiveness of the proposed modules in handling SS-CIL. To assess the effectiveness of the proposed methodology, we conducted experiments with extreme cases such as (i) 1-shot exemplar-free SS-CIL, where only one labeled sample per class is available along with unlabeled data, and (ii) imbalance exemplar-free SS-CIL, where the unlabeled data follows imbalanced distributions. The proposed approach effectively tackles these challenging scenarios. 
To This end, our contributions are (i) As a our knowledge this is the first paper in literature to address exemplar-free SS-CIL setting. (ii) We utilized the foundation models to tackle SS-CIL, for this we proposed three components, task-wise adaptive threshold, data-aware weighted cross entropy and exploting unlabeled data for foundation model classifer alignment. (iii) Extensive experiments on various datasets designed for SS-CIL shows the effectiveness of proposed approach, along with experiments on extreme cases like 1-shot exemplar-free SS CIL and imbalance SS-CIL show the effectiveness of proposed approach. In this context, our contributions are as follows: \begin{itemize}
    \item To the best of our knowledge, this is the first paper in the literature to address the exemplar-free SS-CIL setting. 
    \item We leveraged foundation models to tackle SS-CIL, proposing three components: task-wise adaptive threshold, data-aware weighted cross-entropy, and exploiting unlabeled data for foundation model classifier alignment.
    \item Extensive experiments on various datasets designed for SS-CIL demonstrate the effectiveness of the proposed approach. Furthermore, experiments on extreme cases such as 1-shot exemplar-free SS-CIL and imbalance SS-CIL further validate the efficacy of our approach.
\end{itemize}
The rest of the paper is organized as follows: Section~\ref{sec:related_works} briefly discusses related works, Section~\ref{sec:method} presents notations and the proposed methodology for SS-CIL, and Section~\ref{sec:experiments} provides the experimental results. The paper concludes with an ablation study and analysis of the proposed components.

==> introduction-new.tex <==
Recently, incremental or continual learning has emerged as an important research direction due to its wide applicability, especially in real-time scenarios where models need to adapt to new data continuously. 
It addresses the practical limitations of collecting all data at once and potential privacy concerns where only the model and not the training data, is accessible. But the major challenge faced by neural network models when dealing with continuous data stream is catastrophic forgetting, where previously learned knowledge is overwritten as the model adapts to new information.
%One of the major challenge faced in this task is catastrophic forgetting, where previously learned knowledge is overwritten as the model adapts to new information. 
In this work, we address class incremental learning, where the model is initially trained on a set of base classes and is subsequently updated when a new classes (tasks) becomes available. 
Most of the existing works assume that significant amounts of labeled data is available at each task, which is quite restrictive.
It is only recently that researchers have started to address the more challenging and realistic emi-Supervised Class-Incremental Learning (SS-CIL), where the model has access to a large amount of unlabeled data alongside few labeled samples per task.

In this work, we propose a novel framework termed EfeCT (Exemplar FreE and Class and Task Aware) for the challenging SS-CIL task, in a completely exemplar-free setting.
This implies that we do not need access to any examples of the previous classes, thereby avoiding any privacy concerns or requiring storage costs. 
Inspired by the success of Foundation models for many applications which also includes class-incremental learning [], we propose to leverage their generalization capacity for the challenging SS-CIL task. 
Specifically, we build upon the successful two-stage SLCA framework, where the first stage learns good feature representation, and the second stage utilizes the feature mean and variance of the first stage for classifier adjustment. 
We propose three novel modules to adapt the SLCA framework for the SS-CIL task, namely (i) \textit{Task-wise adaptive threshold} to effectively utilize the unlabeled data; (ii) For each task, to address this issue of imbalance in the unlabeled data that surpasses the threshold, we introduced a \textit{data-aware weighted cross-entropy loss} to enhance performance on under-represented classes and (iii) Exploiting the unlabeled data for better classifier alignment.
Extensive experiments conducted on various datasets, including CIFAR-10, CIFAR-100, and ImageNet-Subset, demonstrate the effectiveness of the proposed modules in handling SS-CIL. 
To this end, our contributions are as follows: 
\begin{enumerate}
    \item To the best of our knowledge, this is the first work in the literature to address the exemplar-free SS-CIL setting. 
    \item We leveraged foundation models to address SS-CIL, proposing three novel components: task-wise adaptive threshold, data-aware weighted cross-entropy, and exploiting unlabeled data for foundation model classifier alignment.
    \item Extensive experiments on various datasets designed for SS-CIL demonstrate the effectiveness of the proposed approach. 
    \item Furthermore, experiments on extreme cases such as 1-shot exemplar-free SS-CIL and imbalance SS-CIL further validate the efficacy of our approach.
\end{enumerate}




%Foundation models have recently played a significant role in modern computer vision applications. In a recent study [], these models were employed for CIL also refererd as slow learner for classifier alignment (SLCA). However, directly applying foundation models to SS-CIL setups may not be effective. To analyze the impact of foundation models in SS-CIL, we incorporated the popular threshold-based semi-supervised learning (SSL) approach known as FixMatch[] with SLCA. FixMatch is an algorithm where, if the confidence of unlabeled samples crosses a predefined threshold (typically 0.95), the unlabeled sample is trained with the pseudo-label of that class. While this approach effectively learns from unlabeled data, in the SS-CIL setting, a fixed threshold may not be effective. The number of classes increases with each task, impact the confidence distribution of unlabeled data. To analyze this confidence variation, we plotted the mean of maximum probabilities (MoMP) of unlabeled data after each task across various datasets. This will give us the idea of on an average what is the maximum confidence of unlabeled data. From figure~\ref{fig:momp_vs_tasks} empirically  we observed that the MoMP value reduced as tasks increased. Maintaining a fixed hard threshold may not effectively leverage learning from the unlabeled data in this dynamic setting. Based on this observation we proposed a \textit{task-wise adaptive threshold} to effectively utilize the unlabeled data. 

%Additionally, there is a notable imbalance in the unlabeled data that surpasses the threshold. To address this issue, we introduced a \textit{data-aware weighted cross-entropy loss} to enhance performance on under-represented classes. Furthermore, we exploit the unlabeled data into the foundation model's classifier alignment process, further boosting performance in the context of semi-supervised class incremental learning (SS-CIL). To the best of our knowledge, this is the first work addressing the exemplar-free SS-CIL setting in the literature. It leverages foundation models to effectively tackle the challenges associated with SS-CIL. Extensive experiments conducted on various datasets, including CIFAR-10, CIFAR-100, and ImageNet-Subset, demonstrate the effectiveness of the proposed modules in handling SS-CIL. To assess the effectiveness of the proposed methodology, we conducted experiments with extreme cases such as (i) 1-shot exemplar-free SS-CIL, where only one labeled sample per class is available along with unlabeled data, and (ii) imbalance exemplar-free SS-CIL, where the unlabeled data follows imbalanced distributions. The proposed approach effectively tackles these challenging scenarios. 

The rest of the paper is organized as follows: Section~\ref{sec:related_works} briefly discusses related works, Section~\ref{sec:method} presents notations and the proposed methodology for SS-CIL, and Section~\ref{sec:experiments} provides the experimental results. The paper concludes with an ablation study and analysis of the proposed components.
